All the {\lambda}-Terms are Meaningful for the Infinitary Relational Model

Infinite types and formulas are known to have really curious and unsound behaviors. For instance, they allow to type {\Omega}, the auto- autoapplication and they thus do not ensure any form of normalization/productivity. Moreover, in most infinitary frameworks, it is not difficult to define a type R that can be assigned to every {\lambda}-term. However, these observations do not say much about what coinductive (i.e. infinitary) type grammars are able to provide: it is for instance very difficult to know what types (besides R) can be assigned to a given term in this setting. We begin with a discussion on the expressivity of different forms of infinite types. Then, using the resource-awareness of sequential intersection types (system S) and tracking, we prove that infinite types are able to characterize the order (arity) of every {\lambda}-terms and that, in the infinitary extension of the relational model, every term has a "meaning" i.e. a non-empty denotation. From the technical point of view, we must deal with the total lack of productivity guarantee for typable terms: we do so by importing methods inspired by first order model theory.

==> consumptionFig1.tex <==
\begin{tikzpicture}



  \draw (0,1) node [below right] {$\ju{C}{t: \sSk\! \rew\! T}  \posPr{\,a\ct 1\,} \hspace{0.7cm} (\ju{D_k}{u:S_k}  \posPr{\,a\ct k\,}\; )_{\kK}$
  } ;

  \draw (0,0.5) --++(7.7,0);

  \draw (2.17,0.5) node [below right] {$\ju{C \uplus_{\kK} D_k}{tu:T} \posPr{\,a\,}$ };








\end{tikzpicture}

